Sampling-Based Approximations to Minimum Bayes Risk Decoding for Neural Machine Translation

In NMT we search for the mode of the model distribution to form predictions. The mode and other high-probability translations found by beam search have been shown to often be inadequate in a number of ways. This prevents improving translation quality through better search, as these idiosyncratic translations end up selected by the decoding algorithm, a problem known as the beam search curse. Recently, an approximation to minimum Bayes risk (MBR) decoding has been proposed as an alternative decision rule that would likely not suffer from the same problems. We analyse this approximation and establish that it has no equivalent to the beam search curse. We then design approximations that decouple the cost of exploration from the cost of robust estimation of expected utility. This allows for much larger hypothesis spaces, which we show to be beneficial. We also show that mode-seeking strategies can aid in constructing compact sets of promising hypotheses and that MBR is effective in identifying good translations in them. We conduct experiments on three language pairs varying in amounts of resources available: English into and from German, Romanian, and Nepali.

==> analysis.tex <==
\subsection{Alternative Hypothesis Spaces}




\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/hypspace-quality-one-direction.png}
    \caption{=50 source sentences, 100 translations using each method per source sentence, proportions are plotted. Other direction looks very similar.}
    \label{fig:alternative-hypothesis-spaces}
\end{figure*}



Thus far we have focused on reducing the number of utility calls such that we can explore larger hypothesis spaces. Another way of tackling the problem of finding effective hypothesis spaces is to make use of strategies that are known empirically to produce good translations, like nucleus sampling and beam search. While these strategies will suffer from inadequacies of highly probable translations, and do not faithfully follow the model distribution, we can include them into the hypothesis set \hypset\ along with ancestral samples and rely on MBR to filter out any idiosyncratic hypotheses. We explore constructing the hypothesis space from \one 1,005 ancestral samples (A), \two 405 nucleus sampling using $p=0.7$ (N) and \three the \nbest list obtained from running beam search with a beam size of $4$ (English-German) or $5$ (English-Romanian and English-Nepali).\fnb{Mention length penalty.} We use \mbrcf using the best configuration found in Section~\ref{sec:experiments:coarse-to-fine-mbr}. It is crucial to note that all settings do still make use of ancestral samples to obtain unbiased estimates of expected utility.\fnb{This sentence confused one reviewer about where we obtain samples from (with replacement from N)?} Our results are shown in Table~\ref{tab:alternative-hypothesis-spaces}.


We find that using alternative strategies for forming the hypothesis space can be beneficial for the quality of the resulting translations. In our high-resource language pair we find that re-ordering the \nbest list resulting from beam search already leads to optimal performance among the strategies that we tested. In our medium- and low-resource language pairs it is more beneficial to construct the hypothesis space using sampling. This is in line with the findings of \citet{eikema-aziz-2020-map}, who show that NMT models are lower entropy for higher resource languages and as a result the beam search output is more representative of the learned conditional distributions. An interesting finding is that for all language pairs constructing \hypset\ from nucleus samples alone is sufficient to reach best performance. The balance between random sampling and mode seeking search that nucleus sampling provides seems to be a particularly effective strategy for constructing hypothesis spaces. Combinations of different strategies seem to be mostly dominated by the performance of the best strategy in the set. It is crucial to note that, because expected utility is a robust objective, it never hurts to include additional hypotheses in \hypset{}.\fnb{``never'' too strong?}

\paragraph{Comparison to Beam Search}
We also included results of running beam search decoding alone in Table~\ref{tab:alternative-hypothesis-spaces}, the \textit{de facto} method of decoding in NMT. We find that sampling-based MBR is able to improve upon beam search for all language pairs considered. 
\mbrnn cannot improve the high resource tasks (en-de and de-en), \mbrns can improve in all tasks except en-de, but requires a great deal of computation, and \mbrcf can improve all tasks except en-de with moderate computation.
Once we construct hypothesis spaces more carefully, with the aid of beam search and/or nucleus samples, \mbrcf can improve on all tasks.
For example, using 1,005 ancestral samples for English-German and \mbrcf does not lead to improvements on beam search, but every other strategy of forming the hypothesis space does. In particular, re-ranking the \nbest list obtained from beam search improves upon beam search itself. The results show the strength of the MBR objective: we can always expand our hypothesis space to improve translation quality, something that is not trivial to do using beam search due to the beam search curse.



\definecolor{Gray}{gray}{0.95}
\newcolumntype{a}{>{\columncolor{Gray}}r}

\begin{table}[]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{0.5em}
    \begin{tabular}{ll ar ar ar}
    \toprule
    & &  
     \multicolumn{2}{c}{en-de} &  \multicolumn{2}{c}{en-ro} &  \multicolumn{2}{c}{en-ne}  \\ \cmidrule(r{1pt}){3-4}\cmidrule(r{1pt}){5-6}\cmidrule{7-8}
    MBR & $\bar{\mathcal H}$ & {\scriptsize BEER} & {\scriptsize BLEU} &  {\scriptsize BEER}  & {\scriptsize BLEU}  &  {\scriptsize BEER}  & {\scriptsize BLEU}  \\  \midrule
    NxS & N & 64.3 & 38.0 & 54.9 & 21.4 & 38.9 & 3.6\\
    C2F & N & +1.1 & +1.9 & +0.4 & +0.2 & +0.4 & +0.2\\
     & B & +0.9 & +1.5 & \bf{+0.5} & \bf{+0.5} & +0.5 & \bf{+0.5}\\
     & all & \bf{+1.3} & +2.4 & \bf{+0.5} & +0.4 & \bf{+0.6} & \bf{+0.5}\\
    \midrule
    BS & - & +0.9 & \bf{+2.8} & -0.1 & +0.1 & -0.8 & +0.2\\
    \midrule\midrule
    & &  
     \multicolumn{2}{c}{de-en} &  \multicolumn{2}{c}{ro-en} &  \multicolumn{2}{c}{ne-en}  \\ \cmidrule(r{1pt}){3-4}\cmidrule(r{1pt}){5-6}\cmidrule{7-8}
    MBR & $\bar{\mathcal H}$  &  {\scriptsize BEER}  & {\scriptsize BLEU}  &  {\scriptsize BEER}  & {\scriptsize BLEU}  &  {\scriptsize BEER}  & {\scriptsize BLEU}  \\  \midrule
    NxS & N & 64.8 & 38.7 & 58.5 & 28.0 & 43.1 & 6.3\\
    C2F & N & +0.9 & +1.1 & +0.5 & +0.7 & +0.5 & +0.2\\
     & B & \bf{+1.0} & \bf{+1.5} & \bf{+0.7} & \bf{+1.2} & +0.5 & \bf{+0.9}\\
     & all & \bf{+1.0} & +1.4 & +0.6 & +1.1 & \bf{+0.8} & +0.8\\
    \midrule
    BS & - & +0.5 & +1.2 & -0.0 & +0.8 & -1.0 & +0.4\\    \bottomrule
    \end{tabular}
    \caption{Comparing N-by-S, Coarse-to-Fine and beam search in terms of BEER and BLEU performance. MBR uses BEER as utility. Coarse-to-fine filters the top-50 hypotheses out of various-sized hypothesis spaces using UF-50 as proxy utility. S in N-by-S is set to 13 to roughly match the same amount of computation as C2F-nucleus, based on a 22.2 times speedup of UF-50 compared to BEER-100 measured in previous experiments.}
    \label{tab:comparison-c2f-beam2}
\end{table}











==> data/utilities.tex <==
order task utility beer bleu meteor chrfpp bleurt
0.0 en-de beer 64.29094342390242 36.95883895342991 56.63504298751409 61.34961928364112 {}
0.1 {} bleu 63.31157348369036 37.46133427459919 55.896458759579275 60.164346973841 {}
0.2 {} meteor 62.52343658613592 33.40438238954783 57.796094523407454 60.48660710407545 {}
0.3 {} chrf++ 63.21833898293295 34.90523332771475 56.87776206573732 61.36048449597897 {}
1.0 de-en beer 64.94502282559593 37.987984940072856 39.26432218724599 60.982243456021784 29.668578137211835
1.1 {} bleu 64.29440291030483 38.32790470083964 38.909848836631845 60.266206355978206 27.52138758245967
1.2 {} meteor 63.513164739824624 36.08758505335041 39.73364430742483 59.770734410020744 28.65956757281432
1.3 {} chrf++ 64.4496571674204 37.18449944445498 39.46411379868686 61.488635013406274 28.256896732150114
2.0 en-ro beer 54.77289146178077 20.97792776478325 33.8930855547347 47.756056965215656 {}
2.1 {} bleu 54.37638134815293 21.252326196428157 40.435153354732066 47.35978071400793 {}
2.2 {} meteor 54.4778307520722 20.94251774918008 40.88652304667305 47.74125436338233 {}
2.3 {} chrf++ 54.242531160043455 20.18389782074364 40.297481158169965 47.988519682222666 {}
3.0 ro-en beer 58.37422836145205 27.497511967429844 32.41657844736432 51.980587216123126 -6.861587055741855
3.1 {} bleu 57.756195530318855 27.848137215832534 32.17292137856945 51.395887484681 -9.336079785664596
3.2 {} meteor 57.46683084586986 26.554894148836983 32.8838013880165 51.53048189922362 -7.203381493990772
3.3 {} chrf++ 58.01258782462687 27.079327723469603 32.725259446344495 52.55684041253132 -7.45958649668745
4.0 en-ne beer 38.43881944966094 3.361031207430902 11.003336012386105 26.079327245935332 {}
4.1 {} bleu 34.92376402315651 3.0338082984706194 10.904055524776362 22.703012051046255 {}
4.2 {} meteor 37.260971524572774 3.418319658931775 13.231265755296342 25.276928481330668 {}
4.3 {} chrf++ 36.841448740976375 2.6409544185870577 12.294943562205395 26.643159982429008 {}
5.0 ne-en beer 42.673425364169155 5.9861514973145304 16.9675958724589 31.177371333331745 -110.28896230072012
5.1 {} bleu 39.8678541355733 5.683182489014219 15.060102624395489 28.399539288084238 -117.77346118737114
5.2 {} meteor 40.37910205117816 4.588212123147879 17.282932235716174 30.8003766855082 -114.15365005392736
5.3 {} chrf++ 40.57175292653849 4.788406895705844 17.00894177303646 31.95556496100348 -115.30287123388713
